Discrete Exponential-Family Models for Multivariate Binary Outcomes

Studies that collect multi-outcome data such as tobacco and alcohol use are becoming increasingly common. In principle, multi-outcomes studies investigate the correlations between outcomes, including, causal links and/or joint distributions. Although there are many methods for studying multivariate outcomes, significant limitations regarding scale and interpretation persist. Here we introduce a model based on the exponential-family for discrete binary outcomes that provides a flexible framework for hypothesis testing of multiple binary outcomes in a computationally efficient fashion.

==> Makefile <==
main.docx: main.tex
	pandoc --from=latex --to=docx main.tex -o main.docx --biblatex && \
		libreoffice main.docx &

